A Flexible, Scalable and Efficient Algorithmic Framework for Primal Graphical Lasso

We propose a scalable, efficient and statistically motivated computational framework for Graphical Lasso (Friedman et al., 2007b) - a covariance regularization framework that has received significant attention in the statistics community over the past few years. Existing algorithms have trouble in scaling to dimensions larger than a thousand. Our proposal significantly enhances the state-of-the-art for such moderate sized problems and gracefully scales to larger problems where other algorithms become practically infeasible. This requires a few key new ideas. We operate on the primal problem and use a subtle variation of block-coordinate-methods which drastically reduces the computational complexity by orders of magnitude. We provide rigorous theoretical guarantees on the convergence and complexity of our algorithm and demonstrate the effectiveness of our proposal via experiments. We believe that our framework extends the applicability of Graphical Lasso to large-scale modern applications like bioinformatics, collaborative filtering and social networks, among others.

==> exp_glasso_real1.tex <==
\section{Real Application: Learning Precision graphs for Movie-Movie Similarities}
\textbf{ MovieLens Data Set:} We study an application of the inverse
covariance estimation method on a dataset obtained from a movie
recommendation problem. We use the benchmark MovieLens-1M dataset
available at \url{http://www.grouplens.org/node/12}, which consists of
1M explicit movie ratings by 6,040 users to 3,706 movies. 
The explicit
ratings are on a 5-point ordinal scale, higher values indicative of
stronger user preference for the movie. 
For our experimental purpose we took the first 3207 movies, as per the ordering in the raw-dataset. 
The statistical problem that has received
considerable attention in the literature is that of predicting
explicit ratings for missing user-movie pairs.  Past
studies~\cite{ruslan} have shown that using movie-movie similarities
based on ``who-rated-what'' information is strongly correlated with
how users explicitly rate movies. Thus using such information as user covariates
helps in improving predictions for explicit ratings. Other than using it as covariates,
one can also derive a movie graph where edge weights represents movie similarities that
are based on global ``who-rated-what'' matrix. Imposing sparsity on such a graph is
attractive since it is intuitive that a movie is generally related to only a few other movies. 
This can be achieved through {\OMOD}. Such a graph provides a neighborhood structure
that can also help directly in better predicting explicit ratings. For instance, in predicting
explicit rating $r_{ij}$ by user $i$ on movie $j$, one can use a weighted average of ratings by the user
in the neighborhood of $j$ derived from the movie-movie graph. 
Such neighborhood information can also
be used as a graph Laplacian to obtain better regularization of user factors in matrix
factorization model as shown in \cite{lurecsys09}. Matrix factorization is a popular technique
used to predict explicit ratings in movie recommender problems. These are multiplicative random
effects model that assume the mean rating by user $i$ on movie $j$ (after adjusting for user and
movie main effects) is given by $\M{u}^{'}_{i}\M{v}_j$, where $\M{u}_i$ and $\M{v}_j$ are user and
movie random-effects vectors respectively. Since the number of missing user-movie pairs are large, shrinkage on both user
and item factors is imperative to avoid over-fitting. This is generally accomplished through a Gaussian
prior with zero-mean and diagonal covariance. However, using the movie-movie graph as prior precision
matrix for movie factors may lead to better performance in practice.

Other than providing useful information to predict explicit ratings,
we note that using who-rated-what information also provides
information to study the relationships among movies based on user
ratings. We focus on such an exploratory analysis here but note that
the output can also be used for prediction problems following
strategies discussed above. A complete exploration of such strategies
for prediction purposes in movie recommender applications is involved and
beyond the scope of this paper.

% since 
%the neighborhood models using item-item similarities are widely used 
%in the literature \cite{bell2008scalable} 
We define the sample movie-movie
similarity matrix as follows: for a movie $i$,  
$\B{x}_i$ is the binary indicator vector denoting users who rated movie $i$. The 
similarity between movie $i$ and $j$ is defined as 
$s_{ij} = \frac{\B{x}_i'\B{x}_j}{\sqrt{\sum\limits x_{i,k}\sum\limits x_{j,k}}}.$ 
 
Note that when $i=j$, $s_{ij}=1$; otherwise $0<=s_{ij}<=1$. Also, the 
sample movie-movie similarity matrix $\M{S}$ obtained from $s_{ij}$ is 
symmetric and postive semi-definite.

%The data-set has a time component to it as well --- user movie pairs have a time-tag associated with them. 
%Based on chronological ordering, we restrict ourselves to a time point corresponding to which 
%3207 movies have been observed. 
%The item-item similarity matrix is based on these 3207 movies. 

\subsection{Timing comparisons}\label{sec:timemlens}
As noted earlier,
for this application we use criterion (\ref{eqn-likhd}) in a non-parametric fashion, where our intention is to learn the 
connectivity matrix corresponding to the sparse inverse covariance matrix. 
We will first show timing comparions of our method \pine (the path-seeking version) along with \GL and \sSMACS. 
We see that \pine is the only method that delivers solutions within a very reasonable amount of time --- we use estimated 
precision matrices to learn about the connectivity structure among the items. 

We sorted the absolute values of the off-diagonal entries in $\s$ and took nine equi-spaced 
quantiles in the range $[q_{8}, q_{75}]$ where $q_8$ corresponds to the 8-th percentile 
and $q_{75}$ corresponds to the 75 th quantile of the entries $\{|s_{ij}|\}_{i > j}$. 
%\textbf{Rahul: what are we doing with these quantiles? --- choosing the grid of lambda values!}
We ran \GL for nine $\lambda$ values corresponding to the quantiles above
denoted by $\lambda_{9} > \ldots > \lambda_{1}$. In our example  $\lambda_{9}=0.1621$ and $\lambda_{1} =0.0277$ --- this range covers 
estimated precision matrices that are quite dense. 

%Since simple thresholding of the sample covariance matrix exactly recovers the connected components of the estimated precision matrix\cite{}, 
%we were tempted to use the exact thresholding rule. However we observed that the size of the maximal connected component corresponding to $\lambda_9$ was 3184 (where% $p=3207$). The screening rule did not leverage much mileage in the domain of $\lambda$ values we considered. 

The path versions of both \pine and \GL were used to obtain solutions on the chosen grid of $\lambda$ values. 
The timings are summarized below:
\begin{itemize}
\item \pine produced a path of solutions across the nine $\lambda$ values using warm-starts in a \emph{total} of 6.722 hours. 
\item The path version of \GL on the other hand, could not complete the same task of computing solutions to (\ref{eqn-likhd}) on the same set of nine $\lambda$ values, within two full days.
\item  We also tried to use \sSMACS for this problem, but it took more than 14 hours to compute the solution corresponding to a single value of $\lambda=\lambda_9$.
\end{itemize}

\subsection{Description of the Results}\label{sec:realmlens}
Figure \ref{fig-spy} represents the sparsity structures of the precision graphs obtained from the movie-movie 
similarities. The graph structures are displayed under the Sparse reverse Cuthill-McKee 
ordering\cite{spy-perm}\footnote{For a sparse symmetric matrix $A$ the reverse Cuthill-McKee ordering is 
a permutation $\pi$ such that $A(\pi,\pi)$ tends to have its nonzero elements closer to the diagonal. This is often used for visualizing the sparsity structure of large dimensional graphs} of the precision matrices 
as delivered by our algorithm \pine for three different values of $\lambda$. The presence of a `dot' in the figure represents a non-zero edge weight in the corresponding movie-movie precision graph. 
The percentages of (off-diagonal) non-zeros are presented below each figure. 
The tapering nature of the graphs for larger values of $\lambda$, show that the movies towards the extreme ends of the axes 
tend to be connected to few other movies. These movies tend to be conditionally dependent on very few other movies. 
The higher density of the points towards the center (of the left two figures) show that those movies tend to be connected to a larger number of other movies. 
\begin{figure}[ht]
  \centering
 \begin{psfrags}
% \psfrag{rhoid9}[][ct]{\textsc{(A)} \hspace{.01in} \scriptsize{p=2000} }
 \psfrag{rhoid9}[][b]{\small{percentage zeros: 98.9 }}
\psfrag{ConnCompSizes}[][cb]{\small{$\log_{10}$(Size of Components)}}
 %\includegraphics[width=.31\textwidth,height=3in]{/h0c/rahulm/rahul/Trevor/Graph_lasso/conn_comp/fig_alon_conncomp1.eps}
\includegraphics[width=.31\textwidth,height=2.7in]{figures/MlensSpyrhoid9.eps}
\end{psfrags}
\begin{psfrags}
 \psfrag{BROWNDATA}[][ct]{\textsc{(B)}  \hspace{.01in} \scriptsize{p=4718} }
 \psfrag{RHO}{}
\psfrag{ConnCompSizes}[][cb]{\small{$\log_{10}$(Size of Components)}}
 \psfrag{rhoid7}[][b]{\small{percentage zeros: 98.7 }}
 \includegraphics[width=.31\textwidth,height=2.7in]{figures/MlensSpyrhoid7.eps}
\end{psfrags}
\begin{psfrags}
 \psfrag{NKIDATA}[][ct]{\textsc{(C)}  \hspace{.01in} \scriptsize{p=24281} }
 \psfrag{rhoid6}[][b]{\small{percentage zeros: 97.8 }}
\psfrag{ConnCompSizes}[][cb]{\small{$\log_{10}$(Size of Components)}}
 \includegraphics[width=.31\textwidth,height=2.7in]{figures/MlensSpyrhoid6.eps}
 \end{psfrags}
  \caption{MATLAB {\tt spy} plots under the reverse Sparse reverse Cuthill-McKee ordering of the vertices
 of the sparse precision matrices obtained via \pine, for three different values of the tuning parameters. A dot represents presence of an edge. The percentage of off-diagonal zeros in the matrix are given below each plot.}
\label{fig-spy}
\end{figure}

We now proceed to look at the nature of the edge-structures and how they evolve across varying strengths of the shrinkage 
parameter $\lambda$ for a smaller sub-graph of the precision-graphs produced by \pine.
For a fixed precision matrix, 
a natural sub-set of `interesting' edges among the all-possible $p(p-1)/2$ edges are the ones corresponding to the 
top $K$ absolute values of partial correlation coefficients. 
The nodes corresponding to these $K$ edges and the edges of the precision graph restricted to these top vertices forms a sub-graph of the $p\times p$ precision graph. 
We summed the absolute values of the off-diagonal entries of the precision matrices across the different $\lambda$ values. The (averaged) 
$p(p-1)/2$ values were ordered and the top ten entries were chosen. These represent the partial correlations having 
the maximal strength (on average) across the different $\lambda$ values taken. 
There were 20 vertices corresponding to these top ten partial correlation coefficients. 
Figure \ref{fig-subgraphs} shows the sub-graphs of the movie-movie precision graphs restricted to the selected 20 movies, across different $\lambda$ values.
The edges in these subgraphs provide some obvious and some interesting insights. For instance, consider the sub-graph corresponding to the largest $\lambda$ (highest
sparsity). Part of strong connectivity among movies 0,1,2,3 is expected since 0,1 and 2,3 are sequels. It is interesting to see there is a connection between 0 and 3,
both of which are Sci-fi movies related to aliens. Other connections also reveal interesting patterns, these can be easily investigated using IMDB movie database.
 
\newpage

\begin{comment}
\begin{figure}
  \centering
  \subfloat[\small{\% non-zeros 90.4}]{\label{fig:gull}\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid1.ps}}                
  \subfloat[\small{\% non-zeros 95.0}]{\label{fig:tiger}\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid2.ps}}
  \subfloat[\small{\% non-zeros 97.8}]{\label{fig:mouse}\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid4.ps}} \\
  \subfloat[\small{\% non-zeros 98.3}]{\label{fig:gull}\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid5.ps}}                
  \subfloat[\small{\% non-zeros 98.8}]{\label{fig:tiger}\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid8.ps}}
  \subfloat[\small{\% non-zeros 98.9}]{\label{fig:mouse}\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid9.ps}}
  \caption{Pictures of subgraphs of the precision matrices induced by the 20 movies corresponding to the largest absolute partial correlations (averaged across difefrent $\lambda$ values).} \label{fig:subgraphs}
\end{figure}
\end{comment}


The movie ids--- movie name mapping is given in the follwing table:
\begin{table}[htpb!]
\begin{center}
  \begin{tabular}{| l | l | }     \hline
(0) {\tt PuppetMaster5: TheFinalChapter (1994) }  & (1) {\tt PuppetMaster4 (1993) }  \\ & \\
(2) {\tt Carnosaur3: PrimalSpecies (1996) } & (3) {\tt Carnosaur2(1995) }   \\ & \\
 (4) { \tt Fridaythe13thPartV: ANewBeginning (1985) } & (5) { \tt Fridaythe13thPartVII:TheNewBlood(1988) } \\ & \\
 (6) {\tt Porky'sRevenge (1985) } & (7) { \tt Porky's II: TheNextDay (1983) }\\ & \\
(8) { \tt SororityHouseMassacre (1986) } & (9) { \tt SororityHouseMassacreII (1990) } \\ & \\
 (10)  {\tt PoliceAcademy5: Assignment:MiamiBeach(1988) } & (11) {\tt PoliceAcademy6:CityUnderSiege(1989) } \\ & \\ 
 (12){\tt RockyIV(1985)} & (13) {\tt  RockyIII (1982) } \\ & \\
(14)  {\tt  Hellbound:HellraiserII(1988) } & (15) {\tt  Hellraiser(1987) } \\ & \\ 
 (16) {\tt  CloseShave,A(1995) } & (17) {\tt  WrongTrousers,The (1993) } \\ & \\
 (18) {\tt  Godfather:PartII,The(1974) } & (19) {\tt  Godfather,The(1972) }  \\ \hline
\end{tabular}
\end{center}
\caption{Table showing thenames of the top 20 Movies, appearing in the top twenty strongest partial correlations. It is seen from 
Figure~\ref{fig:subgraphs} that edges often occur between movies and their sequels.} \label{tab:movies}
\end{table}


\begin{comment}
\begin{table}[htpb!]
\begin{center}
  \begin{tabular}{| c | c | }     \hline
[0] {\tt PuppetMaster5: TheFinalChapter (1994) }  & [1] {\tt PuppetMaster4 (1993) }   \\ 
[2] {\tt Carnosaur3: PrimalSpecies (1996) } & [3] {\tt Carnosaur2(1995) } \\
 [4] { \tt Fridaythe13thPartV: ANewBeginning (1985) } & [5] { \tt Fridaythe13thPartVII:TheNewBlood(1988) } \\
 [6] {\tt Porky'sRevenge (1985) } & [7] { \tt Porky's II: TheNextDay (1983) }\\ 
[8] { \tt SororityHouseMassacre (1986) } & [9] { \tt SororityHouseMassacreII (1990) } \\
 [10]  {\tt PoliceAcademy5: Assignment:MiamiBeach(1988) } & [11] {\tt PoliceAcademy6:CityUnderSiege(1989) } \\
 [12]{\tt RockyIV(1985)} & [13] {\tt  RockyIII (1982) } \\ 
[14]  {\tt  Hellbound:HellraiserII(1988) } & [15] {\tt  Hellraiser(1987) } \\
 [16] {\tt  CloseShave,A(1995) } & [17] {\tt  WrongTrousers,The (1993) } \\
 [18] {\tt  Godfather:PartII,The(1974) } & [19] {\tt  Godfather,The(1972) }  
\end{tabular}
\end{center}
\caption{} \label{tab:movies}
\end{table}
\end{comment}












\begin{comment}
[5] "Fridaythe13thPartVII:TheNewBlood(1988)"
[6] "Porky'sRevenge(1985)"
[7] "Porky'sII:TheNextDay(1983)"
[8] "SororityHouseMassacre(1986)"
[9] "SororityHouseMassacreII(1990)"
[10] "PoliceAcademy5:Assignment:MiamiBeach(1988)"
[11] "PoliceAcademy6:CityUnderSiege(1989)"
[12] "RockyIV(1985)"
[13] "RockyIII(1982)"
[14] "Hellbound:HellraiserII(1988)"
[15] "Hellraiser(1987)"
[16] "CloseShave,A(1995)"
[17] "WrongTrousers,The(1993)"
[18] "Godfather:PartII,The(1974)"
[19] "Godfather,The(1972)"
\newpage

\begin{figure}[ht]
\centering
\begin{psfrags}
\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid1.ps}
\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid2.ps}
\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid4.ps} \\
(a) \hspace{1in} (b) \hspace{1in} (c)   \\
\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid5.ps}
\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid8.ps}
\includegraphics[angle=270,totalheight=.4\textheight,width=.32\textwidth]{figures/ML_graph_rhoid9.ps}
% cross out \{6,7,3}
 \end{psfrags}
  \caption{}
\label{fig-subgraphs}
\end{figure}

Futher analysis of the sub-graphs revealed some interesting and some obvious connections among movies. For instance, consider
subgraph given in figure~\ref{fig-subgraphs}(f). 









\begin{figure}[ht]
  \centering
 \begin{psfrags}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid1.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid2.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid3.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid4.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid5.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid6.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid7.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid8.ps}
\includegraphics[angle=270,totalheight=.3\textheight,width=.32\textwidth]{figures/ML_graph_rhoid9.ps}
% cross out \{6,7,3}
 \end{psfrags}
  \caption{}
\label{fig-subgraphs}
\end{figure}
\end{comment}




\begin{comment}




\begin{figure}[ht]
  \centering
 \begin{psfrags}
 %\includegraphics[width=.31\textwidth,height=3in]{/h0c/rahulm/rahul/Trevor/Graph_lasso/conn_comp/fig_alon_conncomp1.eps}
\includegraphics[width=.31\textwidth,height=3in]{figures/ML_graph_rhoid1.ps}
\end{psfrags}
\begin{psfrags}
 \psfrag{BROWNDATA}[][ct]{\textsc{(B)}  \hspace{.01in} \scriptsize{p=4718} }
 \psfrag{RHO}{}
\psfrag{ConnCompSizes}[][cb]{\small{$\log_{10}$(Size of Components)}}
 \psfrag{rhoid7}[][b]{\small{off-diagonal zeros: 98.7 \%}}
% \includegraphics[angle=270,width=.31\textwidth,height=3in]{figures/ML_graph_rhoid2.ps}
 \includegraphics[angle=270,totalheight=.31\textheight,width=3in]{figures/ML_graph_rhoid2.ps}
\end{psfrags}
\begin{psfrags}
 \psfrag{NKIDATA}[][ct]{\textsc{(C)}  \hspace{.01in} \scriptsize{p=24281} }
 \psfrag{rhoid6}[][b]{\small{off-diagonal zeros: 97.8 \%}}
\psfrag{ConnCompSizes}[][cb]{\small{$\log_{10}$(Size of Components)}}
 \includegraphics[width=.31\textwidth,height=3in]{figures/ML_graph_rhoid3.ps} \\
 \includegraphics[width=.31\textwidth,height=3in]{figures/ML_graph_rhoid4.ps}
 \includegraphics[width=.31\textwidth,height=3in]{figures/ML_graph_rhoid5.ps}
 \includegraphics[width=.31\textwidth,height=3in]{figures/ML_graph_rhoid6.ps}
 \end{psfrags}
  \caption{}
\label{fig-subgraphs}
\end{figure}
\end{comment}


